Dream the Impossible: Outlier Imagination with Diffusion Models

Utilizing auxiliary outlier datasets to regularize the machine learning model has demonstrated promise for out-of-distribution (OOD) detection and safe prediction. Due to the labor intensity in data collection and cleaning, automating outlier data generation has been a long-desired alternative. Despite the appeal, generating photo-realistic outliers in the high dimensional pixel space has been an open challenge for the field. To tackle the problem, this paper proposes a new framework DREAM-OOD, which enables imagining photo-realistic outliers by way of diffusion models, provided with only the in-distribution (ID) data and classes. Specifically, DREAM-OOD learns a text-conditioned latent space based on ID data, and then samples outliers in the low-likelihood region via the latent, which can be decoded into images by the diffusion model. Different from prior works, DREAM-OOD enables visualizing and understanding the imagined outliers, directly in the pixel space. We conduct comprehensive quantitative and qualitative studies to understand the efficacy of DREAM-OOD, and show that training with the samples generated by DREAM-OOD can benefit OOD detection performance. Code is publicly available at https://github.com/deeplearning-wisc/dream-ood.

==> quant.tex <==
\textbf{\model significantly improves OOD detection performance.} As shown in the Table \ref{tab:ImageNet_100_results}, we compare our method with the following recent competitive baselines with \textsc{ImageNet-100} as ID, including (1) Maximum Softmax Probability \citep{hendrycks2016baseline, fort2021exploring}, (2) ODIN score \citep{liang2018enhancing}, (3) Energy score \citep{liu2020energy}, (4) GradNorm score~\citep{huang2021importance}, (5) ViM score~\citep{haoqi2022vim}, (6) KNN distance~\citep{sun2022out}, (7)Generalized ODIN~\cite{hsu2020generalized}  and
(8) VOS \citep{du2022unknown} which synthesizes outliers by modeling the ID embeddings as a mixture of Gaussian distribution and sampling from the low-likelihood region of the feature space. All the baseline methods are fine-tuned using the same pre-trained model weights 

==> test_time.tex <==
For OOD detection, we use the output of the logistic regression uncertainty branch for OOD detection. In particular, given a test input $\*x^*$, the OOD uncertainty score from the classifier $f$ is given by:
\begin{align}
    p_\theta(g \mid \*x^*) = \frac{\exp^{- {\theta}_{\mathrm{u}}( E(\*x^*))}}{1+\exp^{- {\theta}_{\mathrm{u}}( E(\*x^*))}}.
    \label{eq:ood_uncertainty}
\end{align}
% \begin{equation}
%     G(\hat{b}):=\left\{\begin{array}{ll}
% 1 & \text { if }-E(\hat{b}) \geq \gamma, \\
% 0 & \text { if }-E(\hat{b})<\gamma,
% \end{array}\right.
% \label{eq:ood_detection}
% \end{equation}

Therefore, one can exercise the common thresholding mechanism to  distinguish
between ID and OOD inputs:
\begin{equation}
    G(\*x^*)=\left\{\begin{array}{ll}
1 & \text { if }p_\theta(g \mid \*x^*)\geq \gamma, \\
0 & \text { if }p_\theta(g \mid \*x^*) <\gamma,
\end{array}\right.
\label{eq:ood_detection}
\end{equation}
where by convention, 1 represents the positive class (ID), and 0 indicates OOD. The threshold $\gamma$ is typically chosen so that a high
fraction of ID data (e.g., 95\%) is correctly classified. 


For model generalization, we measure the model generalization ability in both the in-distribution test data and data with distribution shifts as follows:
\begin{equation}
    \text{Acc.}(\mathcal{X}^*,\mathcal{Y}) = P_{(\*x^*,y)\sim \mathbb{P}_{\text{in}/\text{out}}}(\arg\max f(\*x^*) = y),
    \label{eq:acc_eval}
\end{equation}
where $(\*x^*,y)\sim \mathbb{P}_{\text{out}}$ hold the same label space  as $\mathbb{P}_{\text{in}}$. Our framework \model is summarized in Algorithm~\ref{alg:algo}.

\begin{algorithm}[h]
\SetAlgoLined
\textbf{Input:} ID training data $\mathcal{D}_\text{in}=\left\{\left(\*x_{i}, {\*y}_{i}\right)\right\}_{i=1}^{n}$, initial model parameters $\theta_{\text{align}}$ for the vision-language alignment branch, classification model $\theta_{\text{CE}}$, nonlinear MLP layer $\phi$.
\\
\textbf{Output:} Learned classifier $f_{\text{CE}}(\cdot)$, and OOD detector $G(\cdot)$.\\
\textbf{Phases:} Phase 1: distilling the distribution prior.  Phase 2: synthesizing the inliers and outliers. Phase 3: classifier training. \\
\While{Phase 1}{
        1. Extract token embeddings $\*c$ of the ID label space $\mathcal{C}$.\\
    2.  Learning an aligned vision-language feature space using Equation~\eqref{eq:cosine_loss}. \\
    3. Generate the normalized features $\*r$.
    }
    \While{Phase 2}{
    1. Identify ID samples that are far from $\mathbb{B}_{\text{far}}$ or near the boundary $\mathbb{B}_{\text{near}}$. \\
    2. Synthesize a set of inliers or outliers $V_i$ around each boundary sample $\*x_i \in \mathbb{B}_1\cup\mathbb{B}_2 \cup...\mathbb{B}_C$ using Equation~\eqref{eq:sample}. \\
    3. Accept the outliers/inliers in each $V_i$ with large/small  $k$-NN distances. 
  }
    \While{Phase 3}{
    1. Train the classification model $f_{{\text{CE}}}$ using Equation~\eqref{eq:all_loss}.
    }
  \While{eval}{
  1.  Evaluate model generalization by Equation~\eqref{eq:acc_eval}. \\
  2.  Calculate the OOD score defined in Equation~\eqref{eq:ood_uncertainty}.\\
  3. Perform OOD detection by Equation~\eqref{eq:ood_detection}.
 }
 \caption{\model: Distribution-dependent Data Generation }
 \label{alg:algo}
\end{algorithm}

==> training.tex <==
\label{sec:training}
\textbf{OOD detection.} The final collection of outlier images $\mathcal{X}_{\text{out}}^\prime$ will be used for the binary training objective based on the energy function~\cite{du2022towards}:
\begin{equation}
\begin{aligned}
    \mathcal{L}_\text{uncertainty}&=\mathbb{E}_{\*x^\prime_{\text{out}} \sim \mathcal{X}^\prime_{\text{out}}}\left[-\log \frac{1}{1+\exp ^{\phi(E(f_{\text{CE}}(\*x^\prime_{\text{out}})))}}\right]\\
    &+\mathbb{E}_{\*x \sim \mathbb{P}_\text{in}}\left[-\log \frac{\exp ^{\phi(E(f_{\text{CE}}(\*x)))}}{1+\exp ^{\phi(E(f_{\text{CE}}(\*x)))}}\right],
\end{aligned}
\label{eq:r_open}
\end{equation}
where $\phi(\cdot)$ is a nonlinear MLP function, $E(\cdot)$ denotes the energy function, and $f_{\text{CE}}(\*x)$ denotes the ID logit in the classification model $f_{\text{CE}}$. In other words, the loss function takes both the ID and synthetic outlier images and aims to estimate the level set through the binary cross-entropy loss.

\textbf{Model generalization.} The generated inlier images $\*x^\prime_{\text{in}} \sim \mathcal{X}^\prime_{\text{in}}$ are directly used as the augmented training data $\mathcal{D}^\prime_{\text{in}} = \{(\*x_i^\prime, y_i^\prime)\}_{i=1}^m$ in the classification model $f_{\text{CE}}$.

\textbf{The overall training objective} combines the standard cross-entropy loss, along with an additional loss in terms of uncertainty regularization or data augmentation:
\begin{equation}
    \min _{\theta} \mathbb{E}_{ \mathcal{D}_{\text{in}},\mathcal{D}_{\text{in}}^\prime}~~\mathcal{L}_\text{CE}+\beta \cdot \mathcal{L}_\text{uncertainty},
    \label{eq:all_loss}
\end{equation}
where $\beta$ is the weight of the uncertainty regularization. $\mathcal{L}_\text{CE}$ denotes the cross-entropy loss. We provide ablation studies in Section~\ref{sec:exp_baseline} demonstrating the superiority of our loss function. 
